In defence of metric learning for speaker recognition

The objective of this paper is 'open-set' speaker recognition of unseen speakers, where ideal embeddings should be able to condense information into a compact utterance-level representation that has small intra-speaker and large inter-speaker distance. A popular belief in speaker recognition is that networks trained with classification objectives outperform metric learning methods. In this paper, we present an extensive evaluation of most popular loss functions for speaker recognition on the VoxCeleb dataset. We demonstrate that the vanilla triplet loss shows competitive performance compared to classification-based losses, and those trained with our proposed metric learning objective outperform state-of-the-art methods.

==> resnet.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{ |c|c|c| }
\hline
\textbf{Layer name} & \textbf{VGG-M-40}  & \textbf{Thin ResNet-34}   \\ \hline\hline
conv1 & \makecell{$5 \times 7,96$, stride 2 \\ $ 3 \times 3$, max pool, stride $ 1 \times 2$}  & \makecell{$7 \times 7,16$, stride 2 \\ $ 3 \times 3$, max pool, stride 2}  \\   \hline
%\addlinespace[1.5ex]
conv2 &  \makecell{$5 \times 5,96$, stride 2 \\ $ 3 \times 3$, max pool, stride 2}    & $\begin{bmatrix}  3 \times 3, 16 \\ 3 \times 3, 16 \end{bmatrix} \times 3 $, stride 1         \\\hline
%\addlinespace[1.5ex]
conv3 & $3 \times 3,256$, stride 1 & $\begin{bmatrix}  3 \times 3,32 \\ 3 \times 3,32 \end{bmatrix} \times 4 $, stride 2      \\\hline
%\addlinespace[1.5ex]
conv4 & $3 \times 3,256$, stride 1 & $\begin{bmatrix}  3 \times 3,64 \\ 3 \times 3,64 \end{bmatrix} \times 6 $, stride 2        \\\hline
%\addlinespace[1.5ex]
conv5 &  \makecell{$3 \times 3,256$, stride 1 \\ $ 3 \times 3$, max pool, stride 2}    & $\begin{bmatrix}  3 \times 3,128 \\ 3 \times 3,128 \end{bmatrix} \times 3 $, stride 2       \\\hline
%\addlinespace[1.5ex]
fc &  $ 4 \times 1$, 512, stride 1  &  $ 9 \times 1$, 512, stride 1                  \\ \hline
\end{tabular}
\vspace{2pt}
\caption{Modified VGG-M and ResNet architectures. ReLU and batchnorm layers are not shown.  Each row specifies the number of convolutional filters, their sizes and strides as {\bf size $\times$ size, \# filters, stride}. The output from the fully connected layer is ingested by the pooling layers.}
\label{table:convnet}
\end{table*}
